X-point and divertor filament dynamics from Gas Puff Imaging on TCV

A new Gas Puff Imaging (GPI) diagnostic has been installed on the TCV tokamak, providing two-dimensional insights into Scrape-Off-Layer (SOL) turbulence dynamics above, at and below the magnetic X-point. A detailed study in L-mode, attached, lower single-null discharges shows that statistical properties have little poloidal variations, while vast differences are present in the 2D behaviour of intermittent filaments. Strongly elongated filaments, just above the X-point and in the divertor far-SOL, show a good consistency in shape and dynamics with field-line tracing from filaments at the outboard midplane, highlighting their connection. In the near-SOL of the outer divertor leg, shortlived, high frequency and more circular (diameter $\sim$15 sound Larmour radii) filaments are observed. These divertor-localised filaments appear born radially at the position of maximum density and display a radially outward motion with velocity $\approx$400\,m/s that is comparable to radial velocities of upstream-connected filaments. Conversely, in these discharges ($B\times\nabla B$ pointing away from the divertor), these divertor filaments' poloidal velocities differ strongly from those of upstream-connected filaments. The importance of divertor-localised filaments upon radial transport and profile broadening is explored using filament statistics and in-situ kinetic profile measurements along the divertor leg. This provides evidence that these filaments contribute significantly to electron density profile broadening in the divertor.

==> Headers.tex <==

% pour l'inclusion de figures en eps,pdf,jpg
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{epsfig}
\epstopdfDeclareGraphicsRule{.pdf}{png}{.png}{convert #1 \OutputFile}
\DeclareGraphicsExtensions{.png,.pdf}
\usepackage{pict2e}

% quelques symboles mathematiques en plus
\usepackage{amsmath}
\usepackage{siunitx}
\usepackage{xfrac}
% greek non italic letters
\usepackage{upgreek}

\usepackage{booktabs}
\usepackage{fancyhdr}
\usepackage{diagbox} % for diagonally cut table cells

\sisetup{
   detect-mode,
   detect-family,
   detect-inline-family=math,
}
\usepackage{textcomp}
\usepackage{eurosym}

% on peut ecrire directement les caracteres avec l'accent
% a utiliser sur Linux/Windows
%\usepackage[latin1]{inputenc}
\usepackage[utf8]{inputenc}

% pour l'inclusion de links dans le document 
\usepackage[colorlinks,bookmarks=false,citecolor={black},linkcolor=blue,urlcolor=blue]{hyperref}
\usepackage{caption,todonotes,multirow,amssymb,amsthm,array,makecell,bm}

\usepackage[section]{placeins}
\usepackage{diagbox}
\usepackage[euler]{textgreek}
%autres package
\usepackage[top=2.2cm, bottom=1.8cm, left=2cm, right=2cm]{geometry}
\usepackage{float,wrapfig,subcaption,import,multicol,color}
\usepackage[T1]{fontenc}
\usepackage{pdflscape}
\usepackage[toc,page]{appendix}
\usepackage{tablefootnote}

% BibLaTeX
\usepackage[backend=biber,style=ieee,citestyle=numeric-comp,sorting=none,natbib=true, hyperref=true]{biblatex}
\usepackage{csquotes}
%\bibliographystyle{IEEEtran} % We choose the "plain" reference style
%\bibliography{references} % Entries are in the "refs.bib" file
\addbibresource{references.bib}
\DeclareSourcemap{
  \maps[datatype=bibtex, overwrite=true]{
    \map{
      \step[typesource=misc, typetarget=online]
    }
  }
}

%\def\changemargin#1#2{\list{}{\rightmargin#2\leftmargin#1}\item[]} \let\endchangemargin=\endlist
\newenvironment{changemargin}[2]{%
\begin{list}{}{%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{#1}%
\setlength{\rightmargin}{#2}%
\setlength{\listparindent}{\parindent}%
\setlength{\itemindent}{\parindent}%
\setlength{\parsep}{\parskip}%
}%
\item[]}{\end{list}}


% Caption Setup
\captionsetup{%
  figurename=Fig.,
  tablename=Tab.,
  format=plain, 
  font=small, 
  labelfont=bf
}

\paperheight=297mm
\paperwidth=210mm

\setlength{\textheight}{235mm}
\setlength{\topmargin}{-1.2cm} % pour centrer la page verticalement
%\setlength{\footskip}{5mm}
\setlength{\textwidth}{15cm}
\setlength{\oddsidemargin}{0.56cm}
\setlength{\evensidemargin}{0.56cm}

\pagestyle{plain}



%=======
% quelques abreviations utiles
\def \be {\begin{equation}}
\def \ee {\end{equation}}
%\def \dd  {{\rm d}}
\def \deg  {{$ ^{\circ}$}}

\newcommand{\mail}[1]{{\href{mailto:#1}{#1}}}
\newcommand{\ftplink}[1]{{\href{ftp://#1}{#1}}}

\let\vaccent=\v % rename builtin command \v{} to \vaccent{}
\renewcommand{\v}[1]{\ensuremath{\mathbf{#1}}} % for vectors
\newcommand{\gv}[1]{\ensuremath{\mbox{\boldmath$ #1 $}}} 
% for vectors of Greek letters
\newcommand{\uv}[1]{\ensuremath{\mathbf{\hat{#1}}}} % for unit vector
\newcommand{\abs}[1]{\left| #1 \right|} % for absolute value
\newcommand{\avg}[1]{\left< #1 \right>} % for average
\let\underdot=\d % rename builtin command \d{} to \underdot{}
\renewcommand{\d}[2]{\frac{d #1}{d #2}} % for derivatives
\newcommand{\dd}[2]{\frac{d^2 #1}{d #2^2}} % for double derivatives
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}} 
% for partial derivatives
\newcommand{\pdd}[2]{\frac{\partial^2 #1}{\partial #2^2}} 
% for double partial derivatives
\newcommand{\pdc}[3]{\left( \frac{\partial #1}{\partial #2}
 \right)_{#3}} % for thermodynamic partial derivatives
\newcommand{\ket}[1]{\left| #1 \right>} % for Dirac bras
\newcommand{\bra}[1]{\left< #1 \right|} % for Dirac kets
\newcommand{\braket}[2]{\left< #1 \vphantom{#2} \right|
 \left. #2 \vphantom{#1} \right>} % for Dirac brackets
\newcommand{\matrixel}[3]{\left< #1 \vphantom{#2#3} \right|
 #2 \left| #3 \vphantom{#1#2} \right>} % for Dirac matrix elements
\newcommand{\grad}[1]{\gv{\nabla} #1} % for gradient
\let\divsymb=\div % rename builtin command \div to \divsymb
\renewcommand{\div}[1]{\v{\nabla} \cdot \v{#1}} % for divergence
\newcommand{\curl}[1]{\Vec{\nabla} \times \Vec{#1}} % for curl
\let\baraccent=\= % rename builtin command \= to \baraccent
\renewcommand{\=}[1]{\stackrel{#1}{=}} % for putting numbers above =

\newcommand{\cs}[1]{\langle #1 \rangle}
